Predicting risk of cardiovascular disease using retinal OCT imaging

Cardiovascular diseases (CVD) are the leading cause of death globally. Non-invasive, cost-effective imaging techniques play a crucial role in early detection and prevention of CVD. Optical coherence tomography (OCT) has gained recognition as a potential tool for early CVD risk prediction, though its use remains underexplored. In this study, we investigated the potential of OCT as an additional imaging technique to predict future CVD events. We analysed retinal OCT data from the UK Biobank. The dataset included 612 patients who suffered a myocardial infarction (MI) or stroke within five years of imaging and 2,234 controls without CVD (total: 2,846 participants). A self-supervised deep learning approach based on Variational Autoencoders (VAE) was used to extract low-dimensional latent representations from high-dimensional 3D OCT images, capturing distinct features of retinal layers. These latent features, along with clinical data, were used to train a Random Forest (RF) classifier to differentiate between patients at risk of future CVD events (MI or stroke) and healthy controls. Our model achieved an AUC of 0.75, sensitivity of 0.70, specificity of 0.70, and accuracy of 0.70, outperforming the QRISK3 score (the third version of the QRISK cardiovascular disease risk prediction algorithm; AUC = 0.60, sensitivity = 0.60, specificity = 0.55, accuracy = 0.55). The choroidal layer in OCT images was identified as a key predictor of future CVD events, revealed through a novel model explainability approach. This study demonstrates that retinal OCT imaging is a cost-effective, non-invasive alternative for predicting CVD risk, offering potential for widespread application in optometry practices and hospitals.

==> sections/Figures_caption.tex <==
\section*{Figures}

\begin{figure}[H]
\begin{center}
\includegraphics[width=\textwidth]{figures/Figure1.pdf}
\end{center}
\caption{ STROBE flow chart describing participant inclusion and exclusion criteria applied to define the study cohort.}\label{fig:flow_chart}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{figures/Figure2.pdf}
    \caption{Distribution of age-sex cohort match. The left histogram illustrates the total of \texttt{CVD+} labeled data used solely for the classification task. The middle histogram shows the total of \texttt{CVD-} for the classification task, while the right histogram illustrates \texttt{CVD-} used for the pretraining task.}
    \label{fig:distribution_data}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Figure3.pdf}
    \caption{The provided workflow diagram illustrates the comprehensive process of training the Variational Autoencoder (VAE) and subsequently using it to acquire the latent vectors (upper section). These latent vectors are then combined with metadata and serve as inputs to the Random Forest (RF) classifier (middle section). Finally, we perform an interpretability analysis by perturbing the most relevant features, reconstructing the corresponding image and computing the optical flow between the perturbed reconstructions (lower section). $z_{left}$ represents the latent vector obtained from the training of the VAE for the left eye. $Z_{right}$ corresponds to the latent vector acquired from training the VAE for the right eye. }
    \label{fig:method}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/Figure4.pdf}
    \caption{Comparison of classifier performance in terms of True Positives (TP), True Negatives (TN), False Positives (FP), and False Negatives (FN). Values above the bars represent the corresponding counts for each classifier.}
    \label{fig:cm_all}
\end{figure}

\setcounter{figure}{5}
\setcounter{subfigure}{0}
\begin{subfigure}[H]
\setcounter{figure}{5}
\setcounter{subfigure}{0}
    \centering
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5a.png}
        \caption{BE-MTDT-RF}
        \label{fig:features_be_mtdt}
    \end{minipage}
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{1}
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5b.png}
        \caption{BE-RF}
        \label{fig:features_be}
    \end{minipage}
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{2}
    \centering
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5c.png}
        \caption{LE-MTDT-RF}
        \label{fig:features_le_mtdt}
    \end{minipage}  
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{3}
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5d.png}
        \caption{LE-RF}
        \label{fig:features_le}
    \end{minipage}   
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{4}
    \centering
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5e.png}
        \caption{RE-MTDT-RF}
        \label{fig:features_re_mtdt}
    \end{minipage}  
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{5}
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5f.png}
        \caption{RE-RF}
        \label{fig:features_re}
    \end{minipage}
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{6}
    \centering
    \begin{minipage}[b]{0.35\textwidth}
        \includegraphics[width=\linewidth]{figures/Figure5g.png}
        \caption{MTDT-RF}
        \label{fig:features_mtdt}
    \end{minipage}  
    \hfill
\setcounter{figure}{5}
\setcounter{subfigure}{-1}
    \caption{Calculation of feature importance magnitudes for the seven different classifiers investigated, where each classifier uses different combinations of data data channels/modalities.}
    \label{fig:features_importances}
\end{subfigure}

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.33]{figures/Figure6.png}
    \caption{Global explanations of features from different data modalities/channels which were considered important by the predictive model for separating the \texttt{CVD+} and \texttt{CVD-} groups. Bar plot summarises the relative importance of latent variables from left $(zl)$ and right $(zr)$ eye OCT images and patient metadata, as percentages.}
    \label{fig:total_importances}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/Figure7.pdf}
    \caption{Optical flow maps presented for three differents B-scans for the left eye. The top row corresponds to the 1st B-scan, the middle image for the 64th B-scan while the bottom row depicts the final B-scan. The yellow circles represent the regions that the optical flow maps highlight when modifying the latent variable zl066. The legend includes the names of layer boundaries in the optical coherence tomography images, as follows:  Internal Limiting Membrane; RNFL: Retinal Nerve Fiber Layer; GCL: Ganglion Cell Layer; IPL: Inner Plexiform Layer; INL: Inner Nuclear Layer; OPL: Outer Plexiform Layer;  BMEIS:	Boundary of Myoid and Ellipsoid of Inner Segments; IB\textunderscore OPR:	Inner Boundary of Outer Segment Retinal Pigment Epithelium Complex; IB\textunderscore RPE: Inner Boundary of Retinal Pigment Epithelium; OB\textunderscore RPE: Outer Boundary of Retinal Pigment Epithelium}
    \label{fig:optical_flow}
\end{figure}






==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
This project was funded by the following institutions: The Royal Academy of Engineering INSILEX (grant no. CiET1819$\backslash{19}$) (A.F.F.), UKRI Frontier Research Guarantee INSILICO (grant no. EP/Y030494/1) (R.B., N.R. and A.F.F.) and Consejo Nacional de Humanidades Ciencias y Tecnologías (CONAHCYT) (scholarship no. 766588) (C.M.G). The NIHR Manchester Biomedical Research Centre also funds the work of A.F.F.

==> sections/tables.tex <==
\section*{Tables}

\begin{table}[H]
  \centering
  \renewcommand{\arraystretch}{1.8} % Aumentar el espacio entre filas en un 50%
  \begin{tabular}{p{4cm}p{5cm}p{5cm}}
    \hline
    Characteristics & \texttt{CVD+} & \texttt{CVD-} \\
    \hline
    Number of subjects & 612 & 2234 \\
    Age: Mean (s.d), years & 60.78 (6.47) &  60.78 (6.47)\\
    Sex: F, M \% & 29.74, 70.26 &   29.74, 70.26 \\
    Ethnicity, \% & \parbox[t]{5cm}{
      90.18 White, 4.26 Mixed, 3.93 Asian or Asian British, 0.33 Black or Black British, 0.16 Chinese, 1.15 Other ethnic group} & 
      \parbox[t]{5cm}{      
      89.22 White, 4.25 Mixed, 4.41 Asian or Asian British, 0.82 Black or Black British, 0.49 Chinese, 0.82 Other ethnic group} \\
    BMI: Mean, kg/m\(^2\)  & 28.31 (4.45) &  27.43 (4.33)  \\
    SBP: Mean, mm Hg & 147.26 (19.57) & 145.1 (18.75)\\
    DBP: Mean, mm Hg & 84.75 (10.23) & 83.22 (9.73)\\
    HbA1c: Mean, mmol/mol & 36.52 (4.32) & 36.59 (6.61)\\
    HbA1c: \% & 2.43 & 2.44 \\
    Alcohol consumption: N, P, C, NA \%  &  3.59, 5.72, 90.69, 0 &  3.92, 3.92, 91.83, 0.33\\
    \hline
  \end{tabular}
  \caption{Characteristics of patients in the \texttt{CVD+} and \texttt{CVD-} sets. N, Never. P, Previous. C, Current. NA, Not answer}
  \label{t:data_caracteristics}
\end{table}

\begin{table}[H]
  \centering
  \renewcommand{\arraystretch}{1.4}
  \begin{tabular}{ |p{3cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
    \hline
    \multicolumn{5}{|c|}{Classification metrics} \\
    \hline
    Classifiers & Accuracy & Sensitivity & Specificity & AUC \\
    \hline
    LE-MTDT-RF & 0.68 & 0.69 & 0.68 & 0.72 \\
    RE-MTDT-RF & 0.67 & 0.69 & 0.67 & 0.70 \\
    \textbf{BE-MTDT-RF} & \textbf{0.70} & \textbf{0.70} & \textbf{0.70} & \textbf{0.75} \\
    MTDT-RF & 0.52 & 0.52 & 0.52 & 0.57 \\
    LE-RF & 0.61 & 0.56 & 0.62 & 0.64 \\
    RE-RF & 0.58 & 0.53 & 0.59 & 0.62\\
    BE-RF & 0.64 & 0.57 & 0.65 & 0.67\\
    \hline
  \end{tabular}
  \caption{Predictive analysis of cardiovascular disease (CVD) metrics utilizing UK Biobank data across seven distinct cases.}
  \label{t:metrics}
\end{table}

\begin{table}[H]
  \centering
  \renewcommand{\arraystretch}{1.4}
  \begin{tabular}{ |p{2.5cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
    \hline
    \multicolumn{5}{|c|}{Classification metrics} \\
    \hline
    Modality & Accuracy & Sensitivity & Specificity & AUC-Value \\
    \hline
    \textbf{BE-MTDT-RF} & \textbf{0.70} & \textbf{0.70} & \textbf{0.70} & \textbf{0.75} \\
    QRISK & 0.55 & 0.60 & 0.545 & 0.60\\
    \hline
    \multicolumn{5}{l}{\small{$\chi^2 = 95.72$, $df=1$, $p=1.31 \times 10^{-22}$}} \\
  \end{tabular}
  \caption{Comparison of classification metric results between our model employing both ocular data and metadata (BE-MTDT) and the QRISK algorithm. McNemar’s Test (*$p < 0.005$)}
  \label{t:metrics_qrisk}
\end{table}
